CREATE: Creativity Evaluation of VLMs using the Visual Remote Associates Test

Vision language models (VLMs) are used in creative tasks such as visual storytelling, design ideation, art interpretation, and advertising. Yet we lack principled ways to measure the lateral reasoning of these models compared to human potential. We introduce CREATE, a semi-automatically constructed benchmark containing 155 visual Remote Associates Test problems. These problems require a solver to find an underlying connection among three seemingly dissimilar images. We conduct a human study (N=25) to validate and ground the quality of our benchmark, and evaluate 11 VLMs. Our findings show that most VLMs underperform humans on this task. Our experiments indicate that the associative ability of VLMs depends on the cue concepts provided in the text and does not universally extend to visual puzzles.

==> Sections/appx_figs.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/heatmap.pdf}
    \caption{Puzzles solved by human only, model only, both human and model, or neither under the five prompt settings. We consider a puzzle solved by a human if at least one participant solves it. }
    \label{fig:combined-results}
\end{figure*}

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{Figures/Task1_compressed.pdf}
    \caption{Prompt for intended word recognition with an example (mouse), which requires models to provide five words per image.}
    \label{fig:task1_prompt}
\end{figure*}

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{Figures/Task3_compressed.pdf}
    \caption{Prompt for intended word recognition with cues with an example of one puzzle (mouse, bus, fan), which involves one or two labeled images and provides the intended word in another image within the same puzzle.}
    \label{fig:task3_prompt}
\end{figure*}
